Anomaly Detection Dataset for Industrial Control Systems

Over the past few decades, Industrial Control Systems (ICSs) have been targeted by cyberattacks and are becoming increasingly vulnerable as more ICSs are connected to the internet. Using Machine Learning (ML) for Intrusion Detection Systems (IDS) is a promising approach for ICS cyber protection, but the lack of suitable datasets for evaluating ML algorithms is a challenge. Although there are a few commonly used datasets, they may not reflect realistic ICS network data, lack necessary features for effective anomaly detection, or be outdated. This paper presents the 'ICS-Flow' dataset, which offers network data and process state variables logs for supervised and unsupervised ML-based IDS assessment. The network data includes normal and anomalous network packets and flows captured from simulated ICS components and emulated networks. The anomalies were injected into the system through various attack techniques commonly used by hackers to modify network traffic and compromise ICSs. We also proposed open-source tools, `ICSFlowGenerator' for generating network flow parameters from Raw network packets. The final dataset comprises over 25,000,000 raw network packets, network flow records, and process variable logs. The paper describes the methodology used to collect and label the dataset and provides a detailed data analysis. Finally, we implement several ML models, including the decision tree, random forest, and artificial neural network to detect anomalies and attacks, demonstrating that our dataset can be used effectively for training intrusion detection ML models.

==> acronym.tex <==
% \acrodef{acronym}[short name]{full name}
\acrodef{IC}[IC]{Integrated Circuit}
% \acrodef{svm}[SVM]{Support Vector Machine}
\newacro{svm}[SVM]{Support Vector Machine}
% Example use \ac{IC} for printing "Integrated Circuit (IC), use \ac{IC} again and it will print (IC)"
% For plural use \acp{IC} for short and \aclp{IC} for long.
% For more see: http://ftp.acc.umu.se/mirror/CTAN/macros/latex/contrib/acronym/acronym.pdf

==> author.tex <==
\author{\IEEEauthorblockN{
Student One\IEEEauthorrefmark{1},
Student Two\IEEEauthorrefmark{2}, 
Student Three\IEEEauthorrefmark{3}
}

\IEEEauthorblockA{
School of Innovation, Design and Engineering, M.Sc.Eng Robotics\\
Mälardalens University, Västerås, Sweden\\
Email:
\IEEEauthorrefmark{1}studentOne, 
\IEEEauthorrefmark{2}studentTwo,
\IEEEauthorrefmark{3}studentThree@student.mdh.se
}}

==> preamble.tex <==
% Report template for Mälardalen University
% Original template can be found: 
% https://www.overleaf.com/latex/templates/ieee-bare-demo-template-for-conferences/ypypvwjmvtdf
% Template file structure organised by: Emil Persson
% The following packages should follow the IEEE conference guidelines.

% Swedish language package 
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage[swedish,english]{babel}

% Graphics
\usepackage{graphicx, float, subfigure, blindtext}

\newcommand\IEEEhyperrefsetup{
bookmarks=true,bookmarksnumbered=true,%
colorlinks=true,linkcolor={black},citecolor={black},urlcolor={black}%
}

% Preferred hyperref setup, Michael Shell
\usepackage[\IEEEhyperrefsetup, pdftex]{hyperref}

% Maths
\usepackage{mathtools}

% These packages must be at the end
\usepackage[nolist,nohyperlinks]{acronym}
\usepackage{cleveref}
\graphicspath{{images/}}

==> sections/abstract.tex <==
\begin{abstract}
An abstract should summarize the work in brief. Now follows some text that you can remove by writing the sign "\%" in front of the command "blindtext", you can always comment out text you have written using the "\%" command.



\end{abstract}

==> sections/acknowledgement.tex <==
\section*{Acknowledgment}
The authors would like to thank ... for his/her/their help and support during the process of writing this paper. 

==> sections/discussion.tex <==
\section{Discussion}
\label{section:disc}
Here you can discuss your results, limitations and new questions that have arose while doing the work. Depending on the size of this report, you can present discussion and conclusion in one common section or in two separate ones. 

==> sections/keywords.tex <==
\begin{center}
\begin{IEEEkeywords}
Alphabetical, Be, In, Order, Should
\end{IEEEkeywords}
\end{center}

==> sections/method.tex <==
\section{Method}
\label{section:method}
In this section, the method used to find an answer to the research questions should be presented. 

If this report presents results from a literature search, this means providing sufficient information for allowing someone else to repeat the literature search and compare the results. I.e., a search using the phrases a, b, and c, was made in database x, y and z on the date Month Date, Year (e.g., July 31st, 2021). The search resulted in x hits. Then, information on how you chose which works to include in this report should be provided. The references should be used for answering your research questions.

If the work reports on an experiment, this part should provide information about the experimental setup, how the experiment was conducted, how data was collected and analyzed etc. Motivate methodological choices through references. Also an experiment should be presented with sufficient detail such that it can be repeated by someone else.

==> sections/results.tex <==
\section{Results}
\label{section:results}
This section should present answers to all research questions.

It is normal to have only one results section, but you can create more sections if finding it more appropriate. You can also divide results into subsections. Perhaps you want to refer to some other section, for example (see Section \ref{section:method}). You can also place figures, you should always reference these in the text, see Figure \ref{fig:MDHlogga} for an example of a figure including subfigures. Remember that all figures should have a figure label explaining their content.


\begin{figure}[H]
    \centering
    \subfigure[MDH logo]{
    \label{fig:MDH1}
    \includegraphics[width=.2\columnwidth]{MDHlogga}}
    \qquad
    \subfigure[MDH logo]{
    \label{fig:MDH2}
    \includegraphics[width=.2\columnwidth]{MDHlogga}}
    \qquad
    \subfigure[MDH logo]{
    \label{fig:MDH3}
    \includegraphics[width=.2\columnwidth]{MDHlogga}}
    \caption[Short text]{This is a example of multiple figures.}
    \label{fig:MDHlogga}
\end{figure}
